A Survey on Fault-tolerance in Distributed Optimization and Machine Learning

The robustness of distributed optimization is an emerging field of study, motivated by various applications of distributed optimization including distributed machine learning, distributed sensing, and swarm robotics. With the rapid expansion of the scale of distributed systems, resilient distributed algorithms for optimization are needed, in order to mitigate system failures, communication issues, or even malicious attacks. This survey investigates the current state of fault-tolerance research in distributed optimization, and aims to provide an overview of the existing studies on both fault-tolerant distributed optimization theories and applicable algorithms.

==> table.tex <==

\begin{table}
\caption{This is my table.} \label{tab:results}
\begin{center}
\begin{tabular}{ll} \hline
naive Bayes & 95.6$\pm$0.15 \\
ID3 & 82.6$\pm$1.2 \\ \hline
\end{tabular}
\end{center}
\end{table}

